A Broad Study of Pre-training for Domain Generalization and Adaptation

Deep models must learn robust and transferable representations in order to perform well on new domains. While domain transfer methods (e.g., domain adaptation, domain generalization) have been proposed to learn transferable representations across domains, they are typically applied to ResNet backbones pre-trained on ImageNet. Thus, existing works pay little attention to the effects of pre-training on domain transfer tasks. In this paper, we provide a broad study and in-depth analysis of pre-training for domain adaptation and generalization, namely: network architectures, size, pre-training loss, and datasets. We observe that simply using a state-of-the-art backbone outperforms existing state-of-the-art domain adaptation baselines and set new baselines on Office-Home and DomainNet improving by 10.7\% and 5.5\%. We hope that this work can provide more insights for future domain transfer research.

==> main <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{bai2021transformers}
Bai, Y., Mei, J., Yuille, A.L., Xie, C.: Are transformers more robust than
  {CNN}s? In: Advances in Neural Information Processing Systems (NeurIPS).
  vol.~34 (2021)

\bibitem{bao2022beit}
Bao, H., Dong, L., Piao, S., Wei, F.: {BE}it: {BERT} pre-training of image
  transformers. In: International Conference on Learning Representations
  (2022), \url{https://openreview.net/forum?id=p-BhZSz59o4}

\bibitem{bashkirova2021visda}
Bashkirova, D., Hendrycks, D., Kim, D., Mishra, S., Saenko, K., Saito, K.,
  Teterwak, P., Usman, B.: Visda-2021 competition universal domain adaptation
  to improve performance on out-of-distribution data. arXiv preprint
  arXiv:2107.11011  (2021)

\bibitem{beery2020iwildcam}
Beery, S., Cole, E., Gjoka, A.: The iwildcam 2020 competition dataset. arXiv
  preprint arXiv:2004.10340  (2020)

\bibitem{ben2010theory}
Ben-David, S., Blitzer, J., Crammer, K., Kulesza, A., Pereira, F., Vaughan,
  J.W.: A theory of learning from different domains, vol.~79. Springer (2010)

\bibitem{bhushan2018deepjdot}
Bhushan~Damodaran, B., Kellenberger, B., Flamary, R., Tuia, D., Courty, N.:
  Deepjdot: Deep joint distribution optimal transport for unsupervised domain
  adaptation. In: European Conference on Computer Vision (ECCV). pp. 447--463
  (2018)

\bibitem{caron2020unsupervised}
Caron, M., Misra, I., Mairal, J., Goyal, P., Bojanowski, P., Joulin, A.:
  Unsupervised learning of visual features by contrasting cluster assignments.
  In: Advances in Neural Information Processing Systems (NeurIPS). vol.~33, pp.
  9912--9924 (2020)

\bibitem{caron2021emerging}
Caron, M., Touvron, H., Misra, I., J{\'e}gou, H., Mairal, J., Bojanowski, P.,
  Joulin, A.: Emerging properties in self-supervised vision transformers. In:
  IEEE International Conference on Computer Vision (ICCV). pp. 9650--9660
  (2021)

\bibitem{changpinyo2021conceptual}
Changpinyo, S., Sharma, P., Ding, N., Soricut, R.: Conceptual 12m: Pushing
  web-scale image-text pre-training to recognize long-tail visual concepts. In:
  IEEE Conference on Computer Vision and Pattern Recognition (CVPR). pp.
  3558--3568 (2021)

\bibitem{chen2020simple}
Chen, T., Kornblith, S., Norouzi, M., Hinton, G.: A simple framework for
  contrastive learning of visual representations. In: International Conference
  on Machine Learning (ICML). pp. 1597--1607. PMLR (2020)

\bibitem{dosovitskiy2021an}
Dosovitskiy, A., Beyer, L., Kolesnikov, A., Weissenborn, D., Zhai, X.,
  Unterthiner, T., Dehghani, M., Minderer, M., Heigold, G., Gelly, S.,
  Uszkoreit, J., Houlsby, N.: An image is worth 16x16 words: Transformers for
  image recognition at scale. In: International Conference on Learning
  Representations (ICLR) (2021),
  \url{https://openreview.net/forum?id=YicbFdNTTy}

\bibitem{dosovitskiy2015discriminative}
Dosovitskiy, A., Fischer, P., Springenberg, J.T., Riedmiller, M., Brox, T.:
  Discriminative unsupervised feature learning with exemplar convolutional
  neural networks. IEEE Transactions on Pattern Analysis and Machine
  Intelligence (TPAMI)  \textbf{38}(9),  1734--1747 (2015)

\bibitem{ganin2017domain}
Ganin, Y., Ustinova, E., Ajakan, H., Germain, P., Larochelle, H., Laviolette,
  F., Marchand, M., Lempitsky, V.: Domain-adversarial training of neural
  networks. Journal of Machine Learning Research (JMLR)  \textbf{17}(1),
  2096--2030 (2016)

\bibitem{gidaris2018unsupervised}
Gidaris, S., Singh, P., Komodakis, N.: Unsupervised representation learning by
  predicting image rotations. arXiv preprint arXiv:1803.07728  (2018)

\bibitem{goodfellow2014explaining}
Goodfellow, I.J., Shlens, J., Szegedy, C.: Explaining and harnessing
  adversarial examples. arXiv preprint arXiv:1412.6572  (2014)

\bibitem{gulrajani2021in}
Gulrajani, I., Lopez-Paz, D.: In search of lost domain generalization. In:
  International Conference on Learning Representations (2021),
  \url{https://openreview.net/forum?id=lQdXeXDoWtI}

\bibitem{he2020momentum}
He, K., Fan, H., Wu, Y., Xie, S., Girshick, R.: Momentum contrast for
  unsupervised visual representation learning. In: IEEE Conference on Computer
  Vision and Pattern Recognition (CVPR). pp. 9729--9738 (2020)

\bibitem{he2016deep}
He, K., Zhang, X., Ren, S., Sun, J.: Deep residual learning for image
  recognition. In: IEEE Conference on Computer Vision and Pattern Recognition
  (CVPR). pp. 770--778 (2016)

\bibitem{hendrycks2018benchmarking}
Hendrycks, D., Dietterich, T.: Benchmarking neural network robustness to common
  corruptions and perturbations. In: International Conference on Learning
  Representations (2019), \url{https://openreview.net/forum?id=HJz6tiCqYm}

\bibitem{hinton2015distilling}
Hinton, G., Vinyals, O., Dean, J.: Distilling the knowledge in a neural
  network. arXiv preprint arXiv:1503.02531  (2015)

\bibitem{hoffman2014one}
Hoffman, J., Tzeng, E., Donahue, J., Jia, Y., Saenko, K., Darrell, T.: One-shot
  adaptation of supervised deep convolutional models. In: International
  Conference on Learning Representations (ICLR) (2014)

\bibitem{hu2018squeeze}
Hu, J., Shen, L., Sun, G.: Squeeze-and-excitation networks. In: IEEE Conference
  on Computer Vision and Pattern Recognition (CVPR). pp. 7132--7141 (2018)

\bibitem{huang2019unsupervised}
Huang, J., Dong, Q., Gong, S., Zhu, X.: Unsupervised deep learning by
  neighbourhood discovery. arXiv preprint arXiv:1904.11567  (2019)

\bibitem{jia2021scaling}
Jia, C., Yang, Y., Xia, Y., Chen, Y.T., Parekh, Z., Pham, H., Le, Q., Sung,
  Y.H., Li, Z., Duerig, T.: Scaling up visual and vision-language
  representation learning with noisy text supervision. In: International
  Conference on Machine Learning (ICML). pp. 4904--4916. PMLR (2021)

\bibitem{dalib}
Jiang, J., Chen, B., Fu, B., Long, M.: Transfer-learning-library.
  \url{https://github.com/thuml/Transfer-Learning-Library} (2020)

\bibitem{jin2020minimum}
Jin, Y., Wang, X., Long, M., Wang, J.: Minimum class confusion for versatile
  domain adaptation. In: European Conference on Computer Vision (ECCV). pp.
  464--480. Springer (2020)

\bibitem{kim2021cds}
Kim, D., Saito, K., Oh, T.H., Plummer, B.A., Sclaroff, S., Saenko, K.: {CDS}:
  Cross-domain self-supervised pre-training. In: IEEE International Conference
  on Computer Vision (ICCV). pp. 9123--9132 (2021)

\bibitem{koh2021wilds}
Koh, P.W., Sagawa, S., Marklund, H., Xie, S.M., Zhang, M., Balsubramani, A.,
  Hu, W., Yasunaga, M., Phillips, R.L., Gao, I., et~al.: Wilds: A benchmark of
  in-the-wild distribution shifts. In: International Conference on Machine
  Learning (ICML). pp. 5637--5664. PMLR (2021)

\bibitem{kornblith2019better}
Kornblith, S., Shlens, J., Le, Q.V.: Do better {I}mage{N}et models transfer
  better? In: IEEE Conference on Computer Vision and Pattern Recognition
  (CVPR). pp. 2661--2671 (2019)

\bibitem{krishna2017visual}
Krishna, R., Zhu, Y., Groth, O., Johnson, J., Hata, K., Kravitz, J., Chen, S.,
  Kalantidis, Y., Li, L.J., Shamma, D.A., et~al.: Visual genome: Connecting
  language and vision using crowdsourced dense image annotations. International
  Journal of Computer Vision (IJCV)  \textbf{123}(1),  32--73 (2017)

\bibitem{krizhevsky2012imagenet}
Krizhevsky, A., Sutskever, I., Hinton, G.E.: {I}mage{N}et classification with
  deep convolutional neural networks. In: Advances in Neural Information
  Processing Systems (NIPS). vol.~25 (2012)

\bibitem{li2021align}
Li, J., Selvaraju, R., Gotmare, A., Joty, S., Xiong, C., Hoi, S.C.H.: Align
  before fuse: Vision and language representation learning with momentum
  distillation. In: Advances in Neural Information Processing Systems
  (NeurIPS). vol.~34 (2021)

\bibitem{lin2014microsoft}
Lin, T.Y., Maire, M., Belongie, S., Hays, J., Perona, P., Ramanan, D.,
  Doll{\'a}r, P., Zitnick, C.L.: Microsoft {COCO}: Common objects in context.
  In: European Conference on Computer Vision (ECCV). pp. 740--755. Springer
  (2014)

\bibitem{liu2021swin}
Liu, Z., Lin, Y., Cao, Y., Hu, H., Wei, Y., Zhang, Z., Lin, S., Guo, B.: Swin
  transformer: Hierarchical vision transformer using shifted windows. In: IEEE
  International Conference on Computer Vision (ICCV). pp. 10012--10022 (2021)

\bibitem{liu2022convnet}
Liu, Z., Mao, H., Wu, C.Y., Feichtenhofer, C., Darrell, T., Xie, S.: A
  {C}onv{N}et for the 2020s. arXiv preprint arXiv:2201.03545  (2022)

\bibitem{long2018conditional}
Long, M., Cao, Z., Wang, J., Jordan, M.I.: Conditional adversarial domain
  adaptation. In: Advances in Neural Information Processing Systems (NeurIPS).
  pp. 1640--1650 (2018)

\bibitem{long2016unsupervised}
Long, M., Zhu, H., Wang, J., Jordan, M.I.: Unsupervised domain adaptation with
  residual transfer networks. In: Advances in Neural Information Processing
  Systems (NeurIPS). pp. 136--144 (2016)

\bibitem{van2008visualizing}
Van~der Maaten, L., Hinton, G.: Visualizing data using t-{SNE}. Journal of
  Machine Learning Research (JMLR)  \textbf{9}(11) (2008)

\bibitem{noroozi2016unsupervised}
Noroozi, M., Favaro, P.: Unsupervised learning of visual representations by
  solving jigsaw puzzles. In: European Conference on Computer Vision (ECCV).
  pp. 69--84. Springer (2016)

\bibitem{ordonez2011im2text}
Ordonez, V., Kulkarni, G., Berg, T.: Im2text: Describing images using 1 million
  captioned photographs. In: Advances in Neural Information Processing Systems
  (NeurIPS). vol.~24 (2011)

\bibitem{peng2019moment}
Peng, X., Bai, Q., Xia, X., Huang, Z., Saenko, K., Wang, B.: Moment matching
  for multi-source domain adaptation. In: IEEE International Conference on
  Computer Vision (ICCV). pp. 1406--1415 (2019)

\bibitem{radford2021learning}
Radford, A., Kim, J.W., Hallacy, C., Ramesh, A., Goh, G., Agarwal, S., Sastry,
  G., Askell, A., Mishkin, P., Clark, J., et~al.: Learning transferable visual
  models from natural language supervision. In: International Conference on
  Machine Learning (ICML). pp. 8748--8763. PMLR (2021)

\bibitem{russakovsky2015imagenet}
Russakovsky, O., Deng, J., Su, H., Krause, J., Satheesh, S., Ma, S., Huang, Z.,
  Karpathy, A., Khosla, A., Bernstein, M., et~al.: Imagenet large scale visual
  recognition challenge. International Journal of Computer Vision (IJCV)
  \textbf{115}(3),  211--252 (2015)

\bibitem{saenko2010adapting}
Saenko, K., Kulis, B., Fritz, M., Darrell, T.: Adapting visual category models
  to new domains. In: European Conference on Computer Vision (ECCV). pp.
  213--226. Springer (2010)

\bibitem{sagawa2022extending}
Sagawa, S., Koh, P.W., Lee, T., Gao, I., Xie, S.M., Shen, K., Kumar, A., Hu,
  W., Yasunaga, M., Marklund, H., Beery, S., David, E., Stavness, I., Guo, W.,
  Leskovec, J., Saenko, K., Hashimoto, T., Levine, S., Finn, C., Liang, P.:
  Extending the {WILDS} benchmark for unsupervised adaptation. In:
  International Conference on Learning Representations (2022),
  \url{https://openreview.net/forum?id=z7p2V6KROOV}

\bibitem{saito2019semi}
Saito, K., Kim, D., Sclaroff, S., Darrell, T., Saenko, K.: Semi-supervised
  domain adaptation via minimax entropy. In: IEEE International Conference on
  Computer Vision (ICCV) (2019)

\bibitem{saito2020uni}
Saito, K., Kim, D., Sclaroff, S., Saenko, K.: Universal domain adaptation
  through self supervision. arXiv preprint arXiv:2002.07953  (2020)

\bibitem{saito2021tune}
Saito, K., Kim, D., Teterwak, P., Sclaroff, S., Darrell, T., Saenko, K.: Tune
  it the right way: Unsupervised validation of domain adaptation via soft
  neighborhood density. In: IEEE International Conference on Computer Vision
  (ICCV). pp. 9184--9193 (2021)

\bibitem{saito2019strong}
Saito, K., Ushiku, Y., Harada, T., Saenko, K.: Strong-weak distribution
  alignment for adaptive object detection. In: IEEE Conference on Computer
  Vision and Pattern Recognition (CVPR). pp. 6956--6965 (2019)

\bibitem{saito2018maximum}
Saito, K., Watanabe, K., Ushiku, Y., Harada, T.: Maximum classifier discrepancy
  for unsupervised domain adaptation. In: IEEE Conference on Computer Vision
  and Pattern Recognition (CVPR). pp. 3723--3732 (2018)

\bibitem{sharma2018conceptual}
Sharma, P., Ding, N., Goodman, S., Soricut, R.: Conceptual captions: A cleaned,
  hypernymed, image alt-text dataset for automatic image captioning. In:
  Proceedings of the 56th Annual Meeting of the Association for Computational
  Linguistics (Volume 1: Long Papers). pp. 2556--2565 (2018)

\bibitem{simonyan2014very}
Simonyan, K., Zisserman, A.: Very deep convolutional networks for large-scale
  image recognition. arXiv preprint arXiv:1409.1556  (2014)

\bibitem{sun2017revisiting}
Sun, C., Shrivastava, A., Singh, S., Gupta, A.: Revisiting unreasonable
  effectiveness of data in deep learning era. In: IEEE International Conference
  on Computer Vision (ICCV). pp. 843--852 (2017)

\bibitem{tan2019efficientnet}
Tan, M., Le, Q.: Efficientnet: Rethinking model scaling for convolutional
  neural networks. In: International Conference on Machine Learning (ICML). pp.
  6105--6114. PMLR (2019)

\bibitem{tang2020unsupervised}
Tang, H., Chen, K., Jia, K.: Unsupervised domain adaptation via structurally
  regularized deep clustering. In: IEEE Conference on Computer Vision and
  Pattern Recognition (CVPR). pp. 8725--8735 (2020)

\bibitem{touvron2021training}
Touvron, H., Cord, M., Douze, M., Massa, F., Sablayrolles, A., J{\'e}gou, H.:
  Training data-efficient image transformers \& distillation through attention.
  In: International Conference on Machine Learning (ICML). pp. 10347--10357.
  PMLR (2021)

\bibitem{tsai2019domain}
Tsai, Y.H., Sohn, K., Schulter, S., Chandraker, M.: Domain adaptation for
  structured output via discriminative patch representations. In: IEEE
  International Conference on Computer Vision (ICCV). pp. 1456--1465 (2019)

\bibitem{tzeng2014deep}
Tzeng, E., Hoffman, J., Zhang, N., Saenko, K., Darrell, T.: Deep domain
  confusion: Maximizing for domain invariance. arXiv preprint arXiv:1412.3474
  (2014)

\bibitem{van2018inaturalist}
Van~Horn, G., Mac~Aodha, O., Song, Y., Cui, Y., Sun, C., Shepard, A., Adam, H.,
  Perona, P., Belongie, S.: The inaturalist species classification and
  detection dataset. In: IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR). pp. 8769--8778 (2018)

\bibitem{vaswani2017attention}
Vaswani, A., Shazeer, N., Parmar, N., Uszkoreit, J., Jones, L., Gomez, A.N.,
  Kaiser, {\L}., Polosukhin, I.: Attention is all you need  \textbf{30} (2017)

\bibitem{venkat2020your}
Venkat, N., Kundu, J.N., Singh, D., Revanur, A., et~al.: Your classifier can
  secretly suffice multi-source domain adaptation. In: Advances in Neural
  Information Processing Systems (NeurIPS). vol.~33, pp. 4647--4659 (2020)

\bibitem{venkateswara2017deep}
Venkateswara, H., Eusebio, J., Chakraborty, S., Panchanathan, S.: Deep hashing
  network for unsupervised domain adaptation. In: IEEE Conference on Computer
  Vision and Pattern Recognition (CVPR). pp. 5018--5027 (2017)

\bibitem{wah2011caltech}
Wah, C., Branson, S., Welinder, P., Perona, P., Belongie, S.: The
  {C}altech-{UCSD} birds-200-2011 dataset  (2011)

\bibitem{wang2020progressive}
Wang, S., Chen, X., Wang, Y., Long, M., Wang, J.: Progressive adversarial
  networks for fine-grained domain adaptation. In: IEEE Conference on Computer
  Vision and Pattern Recognition (CVPR). pp. 9213--9222 (2020)

\bibitem{wu2018unsupervised}
Wu, Z., Xiong, Y., Yu, S.X., Lin, D.: Unsupervised feature learning via
  non-parametric instance discrimination. In: IEEE Conference on Computer
  Vision and Pattern Recognition (CVPR). pp. 3733--3742 (2018)

\bibitem{xie2020self}
Xie, Q., Luong, M.T., Hovy, E., Le, Q.V.: Self-training with noisy student
  improves imagenet classification. In: IEEE Conference on Computer Vision and
  Pattern Recognition (CVPR). pp. 10687--10698 (2020)

\bibitem{xie2017aggregated}
Xie, S., Girshick, R., Doll{\'a}r, P., Tu, Z., He, K.: Aggregated residual
  transformations for deep neural networks. In: IEEE Conference on Computer
  Vision and Pattern Recognition (CVPR). pp. 1492--1500 (2017)

\bibitem{xu2018deep}
Xu, R., Chen, Z., Zuo, W., Yan, J., Lin, L.: Deep cocktail network:
  Multi-source unsupervised domain adaptation with category shift. In: IEEE
  Conference on Computer Vision and Pattern Recognition (CVPR). pp. 3964--3973
  (2018)

\bibitem{xu2019larger}
Xu, R., Li, G., Yang, J., Lin, L.: Larger norm more transferable: An adaptive
  feature norm approach for unsupervised domain adaptation. In: IEEE
  International Conference on Computer Vision (ICCV). pp. 1426--1435 (2019)

\bibitem{you2021logme}
You, K., Liu, Y., Wang, J., Long, M.: Logme: Practical assessment of
  pre-trained models for transfer learning. In: International Conference on
  Machine Learning (ICML). pp. 12133--12143. PMLR (2021)

\bibitem{zhang2019bridging}
Zhang, Y., Liu, T., Long, M., Jordan, M.: Bridging theory and algorithm for
  domain adaptation. In: International Conference on Machine Learning (ICML).
  pp. 7404--7413. PMLR (2019)

\bibitem{zhu2019aligning}
Zhu, Y., Zhuang, F., Wang, D.: Aligning domain-specific distribution and
  classifier for cross-domain classification from multiple sources. In:
  Proceedings of the AAAI Conference on Artificial Intelligence. vol.~33, pp.
  5989--5996 (2019)

\end{thebibliography}


==> tables/tab_domainnet_da.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{ Accuracy comparison with existing domain adaptation baselines on Office-Home. (a) The source is selected from the best single source domain adaptation~\cite{peng2019moment}. (b) For multi source adaptation, all the domains except the target domain (5 domains) are used as the source domains. (c) We use the $Real$ domain as the source domain. Simply using \vit-B from the ALBEF~\cite{li2021align} pre-training outperforms the existing domain adaptation baselines by up to 5.5\% on average. * represents the numbers reported in~\cite{venkat2020your,peng2019moment}}
\setlength{\tabcolsep}{4pt}
\resizebox{1.0\textwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\toprule[1.0pt]
\multicolumn{1}{c|}{\multirow{2}{*}{Backbone}} & \multicolumn{1}{c|}{Pre-training} & \multicolumn{1}{c|}{Downstream} & \multirow{2}{*}{Adaptation} & \multicolumn{5}{c|}{Target Domain} & \multirow{2}{*}{AVG} \\
\cline{5-9}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Data} & \multicolumn{1}{c}{Data} &  & In & Cl & Pa & Sk & Qu &  \\
\hline
\hline
\multicolumn{10}{l}{\textbf{(a) Single source domain adaptation baselines}} \\
ResNet-101* & ImageNet-1K & Source + target & ADDA~\cite{tzeng2014deep} & 14.5 & 39.5 & 29.1 & 30.7 & 14.9 & 25.7 \\
ResNet-101* & ImageNet-1K & Source + target & MCD~\cite{saito2018maximum} & 19.6 & 42.6 & 42.6 & 30.8 & 3.8 & 27.9 \\
\hline
\multicolumn{10}{l}{\textbf{(b) Multi source domain adaptation baselines}} \\
ResNet-101* & ImageNet-1K & Multi Source + target & ADDA~\cite{tzeng2014deep} & 11.4 & 47.5 & 36.7 & 33.5 & 14.7 & 28.8 \\
ResNet-101* & ImageNet-1K & Multi Source + target & MCD~\cite{saito2018maximum} & 22.1 & 54.3 & 45.7 & 43.5 & 7.6 & 34.6 \\
ResNet-101* & ImageNet-1K & Multi source + target & DCTN~\cite{xu2018deep} & 23.5 & 48.6 & 48.8 & 47.3 & 7.2 & 35.1 \\
ResNet-101* & ImageNet-1K & Multi source + target & MSDA~\cite{peng2019moment} & 26.0 & 58.6 & 52.3 & 49.5 & 6.3 & 38.5 \\
ResNet-101* & ImageNet-1K & Multi source + target & SImpAI~\cite{venkat2020your} & 26.5 & 66.4 & 56.6 & 55.5 & \textbf{18.9} & 44.8 \\
\hline
ResNet-101* & ImageNet-1K & Source & \xmark & 22.2 & 48.4 & 49.4 & 38.8 & 6.4 & 33.0 \\
ConvNext-XL & ImageNet-22K & Source & \xmark & 29.7 & 67.7 & 62.2 & 55.5 & 11.4 & 45.3 \\
ViT-L & ImageNet-22K & Source & \xmark & 27.3 & 65.5 & 61.3 & 52.1 & 10.2 & 43.3 \\
Swin-L & ImageNet-22K & Source & \xmark & 30.6 & 67.2 & 62.5 & 54.1 & 11.2 & 45.1 \\
ViT-B & ALBEF~\cite{li2021align} & Source & \xmark & \textbf{37.3} & \textbf{73.6} & \textbf{65.3} & \textbf{62.2} & 12.8 &\textbf{50.3} \\ 
% ViT-B & ALBEF~\cite{li2021align} & Source & \xmark & \textbf{37.3} & \textbf{65.3} & \textbf{12.8} & \textbf{73.6} & \textbf{62.2} & \textbf{50.3} \\
\bottomrule[1.0pt]
\end{tabular}}
\label{tab:domainnet_da}
\end{table}



% % Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \caption{Accuracy comparison with existing domain adaptation benchmarks on Office-Home. (a) The source is selected from the best single source domain~\cite{peng2019moment}. (b) For multi source baselines, all the domains  except the target domain (5 domains) are used as the source domains. (c) We use the $Real$ domain as the source domain. We observe that simply using \vit-B from the ALBEF~\cite{li2021align} pre-training outperforms the existing domain adaptation baselines by up to 5.5\% on average. * represents the numbers reported in~\cite{venkat2020your,peng2019moment}}
% \resizebox{1.0\textwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% \toprule[1.0pt]
% \multicolumn{1}{c|}{\multirow{2}{*}{Backbone}} & \multicolumn{1}{c|}{Pre-training} & \multicolumn{1}{c|}{Downstream} & \multirow{2}{*}{Adaptation} & \multicolumn{5}{c|}{Target Domain} & \multirow{2}{*}{AVG} \\
% \cline{5-9}
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{Data} & \multicolumn{1}{c}{Data} &  & In & Pa & Qu & Cl & Sk &  \\
% \hline
% \hline
% \multicolumn{10}{l}{\textbf{(a) Single source domain adaptation baselines}} \\
% ResNet-101* & ImageNet-1K & Source + target & ADDA~\cite{tzeng2014deep} & 14.5 & 29.1 & 14.9 & 39.5 & 30.7 & 25.7 \\
% ResNet-101* & ImageNet-1K & Source + target & MCD~\cite{saito2018maximum} & 19.6 & 42.6 & 3.8 & 42.6 & 30.8 & 27.9 \\
% \hline
% \multicolumn{10}{l}{\textbf{(b) Multi source domain adaptation baselines}} \\
% ResNet-101* & ImageNet-1K & Multi Source + target & ADDA~\cite{tzeng2014deep} & 11.4 & 36.7 & 14.7 & 47.5 & 33.5 & 28.8 \\
% ResNet-101* & ImageNet-1K & Multi Source + target & MCD~\cite{saito2018maximum} & 22.1 & 45.7 & 7.6 & 54.3 & 43.5 & 34.6 \\
% ResNet-101* & ImageNet-1K & Multi source + target & DCTN~\cite{xu2018deep} & 23.5 & 48.8 & 7.2 & 48.6 & 47.3 & 35.1 \\
% ResNet-101* & ImageNet-1K & Multi source + target & MSDA~\cite{peng2019moment} & 26.0 & 52.3 & 6.3 & 58.6 & 49.5 & 38.5 \\
% ResNet-101* & ImageNet-1K & Multi source + target & SImpAI~\cite{venkat2020your} & 26.5 & 56.6 & 18.9 & 66.4 & 55.5 & 44.8 \\
% \hline
% \multicolumn{10}{l}{\textbf{(c) Single source only baselines without adaptation}} \\
% ResNet-101* & ImageNet-1K & Source & \xmark & 22.2 & 49.4 & 6.4 & 48.4 & 38.8 & 33.0 \\
% ConvNext-XL & ImageNet-22K & Source & \xmark & 29.7 & 62.2 & 11.4 & 67.7 & 55.5 & 45.3 \\
% ViT-L & ImageNet-22K & Source & \xmark & 27.3 & 61.3 & 10.2 & 65.5 & 52.1 & 43.3 \\
% Swin-L & ImageNet-22K & Source & \xmark & 30.6 & 62.5 & 11.2 & 67.2 & 54.1 & 45.1 \\
% ViT-B & ALBEF~\cite{li2021align} & Source & \xmark & \textbf{37.3} & \textbf{65.3} & \textbf{12.8} & \textbf{73.6} & \textbf{62.2} & \textbf{50.3} \\
% \bottomrule[1.0pt]
% \end{tabular}}
% \end{table}

==> tables/tab_office_home_da.tex <==
\begin{table}[t]
\caption{ =Accuracy comparison with domain adaptation baselines on Office-Home. (a, c): For single source adaptation, we use the $Real$ domain as the source domain. (b) For multi source adaptation, all the domains except the target domain (3 domains) are used as the source domains. Simply using \convnext-L pre-trained on ImageNet-22K outperforms the existing domain adaptation baselines by up to 10.7\% on average. * represents the numbers reported in~\cite{tang2020unsupervised,venkat2020your}}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{1.0\textwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c|c}
\toprule[1.0pt]
 \multirow{2}{*}{Backbone} & Pre-training  & Downstream  & \multirow{2}{*}{Adaptation} & \multicolumn{3}{c|}{Target Domain} & \multirow{2}{*}{AVG} \\
 \cline{5-7}
 & Data & Data &  & Ar & Cl & Pr &  \\
 \hline
 \hline
\multicolumn{8}{l}{\textbf{(a) Single source domain adaptation baselines}} \\
% \hline
ResNet-50* & ImageNet-1K & Source + Target & DANN~\cite{ganin2017domain} & 63.2 & 51.8 & 76.8 & 63.9 \\
ResNet-50* & ImageNet-1K & Source + Target & CDAN~\cite{long2018conditional} & 70.9 & 56.7 & 81.6 & 69.7 \\
ResNet-50* & ImageNet-1K & Source + Target & AFN~\cite{xu2019larger} & 70.9 & 57.1 & 81.5 & 69.8 \\
ResNet-50* & ImageNet-1K & Source + Target & MDD~\cite{zhang2019bridging} & 72.5 & 60.2 & 82.3 & 71.7 \\
ResNet-50* & ImageNet-1K & Source + Target & SRDC~\cite{tang2020unsupervised} & 76.3 & 57.1 & 85.0 & 72.8 \\
\hline
\multicolumn{8}{l}{\textbf{(b) Multi source domain adaptation baselines}} \\
ResNet-50* & ImageNet-1K & Multi source + Target & MFSAN~\cite{zhu2019aligning} & 72.1 & 62 & 80.3 & 71.5 \\
ResNet-50* & ImageNet-1K & Multi source + Target & SImpAl~\cite{venkat2020your} & 70.8 & 56.3 & 80.2 & 69.1 \\
ResNet-101* & ImageNet-1K & Multi source + Target & SImpAl~\cite{venkat2020your} & 73.4 & 62.4 & 81.0 & 72.3 \\
\hline
% \hline
\multicolumn{8}{l}{\textbf{(c) Single source only baselines without adaptation}} \\
% \hline
ResNet-50* & ImageNet-1K & Source & \xmark  & 53.9 & 41.2 & 59.9 & 46.1 \\
% ResNet-101 & ImageNet-1K & Source & \xmark  & 68.5 & 52.4 & 79.9 & 66.9 \\
\convnext-XL & ImageNet-22K & Source & \xmark & \textbf{85.1} & 74.0 & \textbf{91.4} & \textbf{83.5} \\
\vit-L & ImageNet-22K & Source & \xmark & 84.0 & 73.0 & 89.9 & 82.3 \\
\swin-L & ImageNet-22K & Source & \xmark & 83.4 & \textbf{74.3} & 90.9 & 82.8 \\
\vit-B & ALBEF~\cite{li2021align} & Source & \xmark & 72.5  & 81.7& 87.2 & 80.4 \\
% \multirow{2}{*}{\vit-B} & ImageNet-1K  & \multirow{2}{*}{Source} & \multirow{2}{*}{\xmark} &  \multirow{2}{*}{72.5} & \multirow{2}{*}{81.7} & \multirow{2}{*}{87.2} & \multirow{2}{*}{80.4}  \\
% & + Image-Text data & & & & & & \\
\bottomrule[1.0pt]
\end{tabular}}
\label{tab:office_home_da}
\end{table}



